Capturing Bisimulation-Invariant Exponential-Space Complexity Classes

Otto's Theorem characterises the bisimulation-invariant PTIME queries over graphs as exactly those that can be formulated in the polyadic mu-calculus. This extends to a characterisation of the full bisimulation-invariant exponential-time hierarchy, using a higher-order extension of the polyadic mu-calculus, called PHFL, which is naturally stratified by type order. The bisimulation-invariant fragment of k-EXPTIME is captured by the fragment of PHFL whose formulas have type order at most k. This is obtained using a generalisation of the Immerman-Vardi Theorem by Freire and Martins. Here we provide such a characterisation of the exponential-space hierarchy. We show that the bisimulation-invariant fragment of k-EXPSPACE is captured by the fragment of PHFL of type order k+1 whose formulas are tail-recursive. Tail recursion limits the interplay between fixpoints and higher-order functions so that model checking based on fixpoint iteration can be made more space efficient in a way comparable to tail recursion in programming languages. The capturing result makes use of a generalisation of Vardi's characterisation of PSPACE as first-order logic with partial fixpoints, namely that k-EXPSPACE is captured by higher-order logic of order k+1 with partial fixpoints.

==> eptcsdata.tex <==
\providecommand{\firstpage}{49}
\providecommand{\publicationstatus}{G. Bacci, M. Randour (Eds.): Seventeenth\\
International Symposium on Games, Automata, Logics,\\
and Formal Verification (GandALF 2026)\\
EPTCS 454, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.454.5}{10.4204/EPTCS.454.5}}

